Efficient Real-world Testing of Causal Decision Making via Bayesian Experimental Design for Contextual Optimisation

The real-world testing of decisions made using causal machine learning models is an essential prerequisite for their successful application. We focus on evaluating and improving contextual treatment assignment decisions: these are personalised treatments applied to e.g. customers, each with their own contextual information, with the aim of maximising a reward. In this paper we introduce a model-agnostic framework for gathering data to evaluate and improve contextual decision making through Bayesian Experimental Design. Specifically, our method is used for the data-efficient evaluation of the regret of past treatment assignments. Unlike approaches such as A/B testing, our method avoids assigning treatments that are known to be highly sub-optimal, whilst engaging in some exploration to gather pertinent information. We achieve this by introducing an information-based design objective, which we optimise end-to-end. Our method applies to discrete and continuous treatments. Comparing our information-theoretic approach to baselines in several simulation studies demonstrates the superior performance of our proposed approach.

==> Bayesian experimental design for contextual optimisation/_math.tex <==
% math packages

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{bm}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



\newcommand{\designnet}{\pi_\phi}
\newcommand{\policy}{\pi}
\newcommand{\latent}{\theta}
\newcommand{\critic}{U}
\newcommand{\criticnet}{U_\psi}
\newcommand{\proposal}{q}
\newcommand{\proposalnet}{q_\zeta}

\newcommand{\prior}{p(\latent)}
\newcommand{\priori}[1]{p(\latent_{#1})}

\newcommandx{\histmarg}[1][1=\designnet]{p(h_T| #1)}
\newcommandx{\histlik}[1][1=\designnet]{p(h_T|\latent, #1)}
\newcommandx{\histliki}[2][2=\designnet]{p(h_T|\latent_{#1}, #2)}

\newcommand{\obslik}{p(y|\latent, \xi)}
\newcommand{\obsliki}[1]{p(y_{#1}|\latent, \xi_{#1})}
\newcommand{\obsmarg}{p(y|\xi)}

\newcommand{\obspost}{p(\latent|\xi, y)}


\newcommand{\sPCE}[1]{\mathcal{L}_T({#1}, L)}
\newcommand{\sEIG}[1]{\mathcal{I}_T(#1)}
\newcommand{\grad}{\nabla_{(\phi, \psi)}}



\newcommand{\ppx}[1]{\frac{\partial}{\partial #1}}
\newcommand{\pypx}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddx}[1]{\frac{\partial}{\partial #1}}
\newcommand{\dydx}[2]{\frac{d #1}{d #2}}


\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\newcommand{\iid}{\overset{\scriptstyle{\text{i.i.d.}}}{\sim}}

%%%% shortcuts for the proofs
% \newcommand{\multiple}{\frac{(L+1) \exp(U(h_T,\theta_0)) }{ \exp(U(h_T,\theta_0)) + \sum_{i=1}^L \exp(U(h_T,\theta_i)) }}





% Some specific definitions to us

\newcommand{\Pa}[1]{\text{pa}(#1)} % See usage in notation.tex. Chosen to match Daphne's book.
\newcommand{\Do}[1]{\text{do}(#1)} % See usage in notation.tex. Chosen to match Daphne's book.

\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}






% Some imported defaults

%Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\rvA{{\mathbf{A}}}
\def\rvC{{\mathbf{C}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\bbeta{{\bm{\beta}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\data{\mathcal{D}}

\newcommand{\unconditionaljoint}{p(\rvy, \rvm^* | \rvC, \rvC^*, \Do{\rvA})}
\newcommand{\unconditionaljointzero}{p(\rvy, \rvm^*_0 | \rvC, \rvC^*, \Do{\rvA})}
\newcommand{\conditionaljoint}{p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA}, \psi)}


==> Bayesian experimental design for contextual optimisation/background.tex <==
% \vspace{-5pt}
\section{Problem set-up} % Background + relevant notation and objects (Simulator, regret etc)
% The goal of a causal inference method is to uncover the true \textcolor{red}{structural equations/causal effects}, assuming that the underlying causal graph as known \textcolor{red}{CITE}. 
We are interested in the efficient evaluation of the regret of past treatment assignment decisions.
We formalise this by considering a contextual optimisation problem in which treatment, $\rva$, is applied in context, $\rvc$, to receive reward $y$.
% We denote the context as $\rvc$, the treatment (or action) as $\rva$ and the reward as $y$.
% We can think of $\rvc$ as a set of relevant but \emph{unchangeable} attributes, and of $\rva$ as a set of actions that we apply to that context.
For example, in the customer engagement scenario, $\rvc$ would be the information we have about the customer that cannot be directly acted upon, such as age, income and historical data of past interactions, $\rva$ would denote a particular choice of promotions that we offer to the customer, and the reward $y$ would be the future revenue generated by the customer, net of promotion costs. 

% Actions may in general be either discrete or continuous.
%%  In causal inference, the evaluation task is of particular importance.

\paragraph{Expected regret}  We are interested in gathering data to evaluate the \emph{expected regret} of the past action $\rva$ performed in a context of interest $\rvc^*$. This is defined as
%\vspace{-10pt}
\begin{equation}
    R(\rva, \rvc^*) = m(\rvc^*) -  \E[y|\Do{\rva},\rvc^*], \label{eq:regret}
\end{equation}
where $p(\cdot|\Do{\rva},\rvc^*)$ denotes the interventional distribution when action $\rva$ is applied to context $\rvc^*$ and $m(\rvc^*) = \max_{\rva^{\prime}} \E[y | \Do{\rva^{\prime}},\rvc^*]$ denotes the best obtainable outcome for context $\rvc^*$.
Suppose that $\rva$ has been performed historically to $\rvc^*$, and we wish evaluate the regret of this treatment. 
The primary obstacle to evaluating this regret in the real world is that $m(\rvc^*)$ is not known, i.e.~we do not know how much better the outcome could have been if a different treatment had been applied. % (Adam: stopping here)
We therefore wish to obtain experimental data, possibly from different contexts, that will help us to efficiently infer $m(\rvc^*)$.
Gathering data to learn $m(\rvc^*)$ also aids in choosing the best treatment in \emph{future} interactions with $\rvc^*$.
% In addition to ..., wish that the data obtained through experimentation can help us choose better treatments in the future, namely those that realize the highest possible reward under the context of interest, $m(\rvc^*)$, or equivalently---minimizing the regret.

% We define the maximum function as the maximum obtainable reward for a given context 
% % We define $m: \text{Context space} \rightarrow \R$ to be the function mapping context $\rvc$ to the maximum obtainable reward  
% \begin{equation}
%     m(\rvc) = \max_\rva \E[y | \Do{\rva},\rvc].
% \end{equation}


% \subsection{A Bayesian experimental design view on model evaluation and model improvement}
% The goal of our experimental design process is twofold. % We wish to obtain data that can help us make better future decisions 
% Firstly, we are interested in \emph{evaluating a model}, specifically evaluating the regret of a certain set of treatments $\rva^*$ that were applied in some contexts of interest $\rvc^*$. 
% Secondly, we are interested in \emph{obtaining data} that can help us to make better decisions in future. 
% Secondly, wish that the data obtained through experimentation can help us choose better treatments in the future, namely those that realize the highest possible reward under the context of interest, $m(\rvc^*)$, or equivalently---minimizing the regret.
% We formulate this problem mathematically as collecting data that helps us to learn the maximum function $m(\rvc)$. 
% A related objective for non-contextual optimization was introduced in Maximum Entropy Search \citep{wang2017max}.


\paragraph{Bayesian model} In general, we also do not know the true interventional distribution $p(y | \Do{\rva}, \rvc)$.
We therefore model the relationship between $\rva,\rvc$ and $y$ is a Bayesian manner, by introducing a Bayesian parameter $\psi$ with a prior $p(\psi)$.
Different samples of $\psi$ corresponds to different hypotheses $p(y|\text{do}(\rva),\rvc,\psi)$, whilst marginalising over $\psi$ summarises the total Bayesian uncertainty in $y|\text{do}(\rva),\rvc$.
Figure~\ref{fig:stylized_example} illustrates an example with a binary treatment.
% Our requirement for the model is that a sample $y$ of $p(y|\Do{\rva},\rvc,\psi)$ be differentiable w.r.t. $\rva$.



% that describes different possible joint distributions. 
% Let $\psi \sim p(\psi|\mathcal{D})$ represent the posterior distribution given existing observational data.
% Our simulator model provides predictions for $p(y|\text{do}(\rva),\rvc,\psi)$. 
% By sampling different realisations of $\psi$, we can compute our Bayesian uncertainty in possible outcomes $y$ for different contexts $\rvc$ and different actions $\rva$, as well as possible values of $m(\rvc^*)$. 
%% We assume y is cts? .

\paragraph{The role of causality} 
Causal considerations are central to building a correct model of the interventional distribution $p(y|\Do{\rva},\rvc)$, particularly when the prior $p(\psi)$ is fitted by conditioning on past \emph{observational} data.
By making certain assumptions about the causal graph and the (non-)existence of unobserved confounders, one can reduce the problem to that of learning specific functions \citep{pearl2009causal,sharma2021dowhy}.
These assumptions are often made implicitly in the optimisation literature \citep{bareinboim2015bandits}.
Through suitable assumptions, any Bayesian model that predicts $y$ from $\rva,\rvc$ can be used as a model for $p(y|\Do{\rva},\rvc)$, so a causal treatment of the problem does not restrict the class of models that can be considered.
Alternatively, the Bayesian parameter $\psi$ can incorporate uncertainty in the causal graph \citep{heckerman1999bayesian,annadani2021variational,geffner2022deep}.
Our approach to experimental design is concordant with either of these modelling choices.



% \paragraph{Move some of this into the caption and remove rest}
% Figure~\ref{fig:stylized_example} gives a stylized example of a binary treatment case, assuming the outcomes $y$ are caused by the context $\rvc$ and treatments $\rva$. In this case the interventional distribution equals the conditional, $p(y | \Do{\rva}, \rvc) = p(y | \rva, \rvc)$.  Given a realisation of $\psi$ and an action $\rva  \in \{1, 2\}$, the reward is $y = f_{\psi, \rva}(\rvc)$---a deterministic quadratic function of $\rvc$; similarly, given $\psi$ and $\rva$, the max-value $m(\rvc^*)$ is a deterministic function of $\rvc^*$. The dark (resp. light) shaded area shows our uncertainty about $f_{\psi, \rva}$ arising from uncertainty in $\psi$, measured by one (resp. two) standard deviations from the mean. 



%ample different $\psi$  Our Bayesian simulator 
%TODO explain. 

% \textbf{Example.} This could be the place to introduce single confounding root and a simple example purely with functional uncertainty. Need to make people feel sure that the do-notation is not scary. One or two concrete examples here would be v useful. (You do not need to go super explicitly, just get to the fact that $\psi$ can be (the parameters of) a simple function, assuming SCR graph.


% \paragraph{Bayesian Experimental Design (BED)}
% BED \citep{lindley1956} is a principled information-theoretic framework for designing optimal experiments to learn about \emph{model parameters}~$\theta$. Starting with a prior $p(\theta)$ and observation likelihood given parameters and designs $p(y | \theta, \xi)$, the optimal design is the one maximising the expected information gain (EIG), also equivalent to the mutual information between $\theta$~and~$y$, $I(\xi) = \E_{p(\theta)p(y | \theta, \xi)}\left[ \log \frac{p(y | \theta, \xi)}{p(y | \xi)} \right]$.
% \begin{equation}
%     I(\xi) = \E_{p(\theta)p(y | \theta, \xi)}\left[ \log \frac{p(y | \theta, \xi)}{p(y | \xi)} \right].
% \end{equation}
% Given a Bayesian model for the parameters and the observation likelihood, the optimal experiment $\xi$ is the one maximising the expected information gain (EIG)   

==> Bayesian experimental design for contextual optimisation/conclusion.tex <==
\vspace{-10pt}
\section{Discussion and Conclusion}
By combining ideas from Bayesian experimental design, contextual bandits and Bayesian optimisation, we proposed a method for real-world model testing by regret evaluation of past context-dependent treatment assignments. 
Our method also applies to gathering data to improve future decision making, in fact, we saw that gaining information for regret evaluation and for model improvement are really two sides of the same coin.
% Unfortunately, regret is unknown in the real world since we cannot observe the maximum achievable rewards.
% However, by collecting data for testing purposes, our method can both accurately estimate regret and help us make better decisions in the future.
To compute large batch designs efficiently, we cast the problem in terms of implicit likelihood BED, resulting in a model agnostic approach that is able to handle both discrete and continuous designs.

% There are several avenues for future work. The first one is making our method more practical, for example, 
Future work may introduce the ability to handle constraints, and explore the scaling of our method to high dimensional treatments and contexts, both continuous and discrete.
Our method could also be extended to apply to sequential, adaptive experimentation. % with
% The second one would involve improving and extending the method, for example to sequential settings. Finally, we would like to apply our approach to a wider range of problems, both semi-synthetic and real-world. 

==> Bayesian experimental design for contextual optimisation/experiments.tex <==
\section{Empirical Evaluation}

\begin{wrapfigure}[7]{r}{0.29\textwidth}
\vspace{-25pt}

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp18011062446716308] 
\draw   (123.38,152.05) .. controls (129.18,146.14) and (138.68,146.06) .. (144.59,151.86) .. controls (150.5,157.67) and (150.59,167.16) .. (144.78,173.07) .. controls (138.98,178.98) and (129.48,179.07) .. (123.57,173.27) .. controls (117.66,167.46) and (117.57,157.96) .. (123.38,152.05) -- cycle ;
%Shape: Circle [id:dp6837916909787485] 
\draw   (76.09,200.92) .. controls (81.9,195.01) and (91.39,194.92) .. (97.3,200.73) .. controls (103.21,206.53) and (103.3,216.03) .. (97.5,221.94) .. controls (91.69,227.85) and (82.19,227.94) .. (76.28,222.13) .. controls (70.37,216.33) and (70.29,206.83) .. (76.09,200.92) -- cycle ;
%Shape: Circle [id:dp6401485336578827] 
\draw   (26.86,152.58) .. controls (32.66,146.67) and (42.16,146.58) .. (48.07,152.38) .. controls (53.98,158.19) and (54.07,167.69) .. (48.26,173.6) .. controls (42.46,179.51) and (32.96,179.59) .. (27.05,173.79) .. controls (21.14,167.98) and (21.06,158.49) .. (26.86,152.58) -- cycle ;
%Straight Lines [id:da41994824421442045] 
\draw    (116.25,162.24) -- (52.76,162.24) ;
\draw [shift={(119.25,162.24)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da8453011583604917] 
\draw    (48.26,173.6) -- (73.95,198.82) ;
\draw [shift={(76.09,200.92)}, rotate = 224.48] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da34542389820566943] 
\draw    (123.57,173.27) -- (99.38,198.56) ;
\draw [shift={(97.3,200.73)}, rotate = 313.73] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
% Text Node
\draw (37.56,163.09) node    {$\rvc$};
% Text Node
\draw (134.08,162.56) node    {$\rva$};
% Text Node
\draw (86.79,211.43) node    {$y$};


\end{tikzpicture}
\caption{
Causal graph.
%An example of a causal graph. Adam: I'm not sure this graph is super useful here. What we do need is to explain why `causal' is coming in (because interventional distribution). But also explain why some baselines do (UCB) are not usually called causal (because they \emph{only} model the interventional distribution. Also, in experiments, we should draw the single confounding root graph and make clear it's not a limitation of our method, but a simple choice we made for the workshop paper experiments.
}
\label{fig:scr_graph}
\end{wrapfigure}
We test the efficacy of our method on several synthetic experiments. % for which we know the true contextual max-values $\rvm^*$.
In all synthetic experiments, we assume the causal graph is as shown in Figure~\ref{fig:scr_graph}, but note that our method is not restricted to this graph structure. %: the outcome is caused by the treatment and the context, and the treatment cannot affect the context.
% \paragraph{Baselines} 
We compare our method against random treatment assignment and the Upper Confidence Bound (UCB) \citep{auer2002using} algorithm. % The UCB of an action $\rva$ in context $\rvc$ at level $\gamma$ is
% $\text{UCB}_\gamma(\rva; \rvc)  = \E[y | \rva, \rvc ] + \gamma \sqrt{\text{Var}(y | \rva, \rvc )}$, and the optimal action is the one maximizing it. 
% We approximate $\text{UCB}_\gamma(\rva; \rvc)$ using samples. %We approximate the mean and the standard deviation using samples, and when actions are continuous we evaluate $\text{UCB}_\gamma$ on a grid.
% The treatment selected under UCB at  level % $\alpha$ is $\text{UCB}_\alpha [\E[y | \rva, \rvc ] + \alpha \sqrt{(Var[y | ])} ]$.
%We approximate the expectations with samples from $p(\psi)$ 
% \paragraph{Evaluation metrics}  
Our key evaluation metrics are \textbf{EIG} and \textbf{accuracy} of inferring $\rvm^*$. For the former we evaluate~\eqref{eq:infonce_bound} with the trained critic and learnt designs. For the latter, we sample a realisation $\tilde{\psi}$ and $\tilde{\rvm}^*$ from the prior, treating it as the ground truth environment in the Deployment stage of our framework (\S~\ref{sec:deployment}). 
We report the mean squared error (MSE) between our estimate $\rvm^*$ and the ground truth $\tilde{\rvm}^*$. We report three additional metrics---average regret, MSE of estimating $\tilde{\psi}$, and deviation from the true optimal treatment. Full details about the models, training, and further results are given in Appendix~\ref{sec:appendix_experiments}.


\begin{figure}[t]
  \vspace{-15pt}
  \centering
  \includegraphics[width=0.92\textwidth]{fig/figure1_AB.pdf}
\vspace{-15pt}
\caption{Discrete treatments: optimal designs and key metrics. More details in Appendix~\ref{sec:appendix_experiments}. %Our method chooses treatments that will be most informative about the maximum values at the test contexts.
\vspace{-20pt}
}
\label{fig:exp_discrete_ab}
\end{figure}
\paragraph{Discrete treatments}
% \paragraph{Four treatments and quadratic reward}
We consider a model with four treatment options, two of which are \emph{a priori} sub-optimal; the other two have the same mean but Treatment 1 has higher variance than Treatment 2 (Figure~\ref{fig:exp_discrete_ab}).
% Our method has learnt the intuitively optimal strategy, name
Intuitively, the optimal strategy would be to A/B test only the top 2 treatments, which is exactly what our method has learnt. The random method is wasteful as it queries the sub-optimal treatments, while $\text{UCB}_1$ only ever queries Treatment 1. As a result, our method is much more accurate at estimating the true $\rvm^*$.


\paragraph{Continuous treatments}
We test our method on a continuous treatment problem, where we design a batch of 40 experiments to learn about the max-values at 39 evaluation contexts. As Table~\ref{tab:cts_40d_main} shows, our method outperforms the baselines on all metrics. Although our method is optimised to accurately estimate $\tilde{\rvm}^*$, it is also significantly better at estimating $\tilde{\psi}$, which in turn translates to choosing better treatments in the future, as the lower $\text{MSE}(\rvA)$ indicates.
% Vary the design batch from 10 to 100; similar designs to $\text{UCB}_{1.0}$ -- not wasteful. 
% Better treatments -- lower MSE ofro A. 
\begin{table}[t]
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.9} 
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{lccccc}
Method             & EIG estimate      & MSE$(\rvm^*)$       & MSE$(\psi)$       & MSE$(\rvA)$       & Regret    \\
\toprule
Random$_{0.2}$     & 5.407 $\pm$ 0.003 & 0.0041 $\pm$ 0.0001 & 0.0114 $\pm$ 0.0003 & 0.544 $\pm$ 0.023 & 0.091 $\pm$ 0.002 \\
Random$_{1.0}$     & 5.798 $\pm$ 0.004 & 0.0024 $\pm$ 0.0002 & 0.0053 $\pm$ 0.0002 & 0.272 $\pm$ 0.018 & 0.060 $\pm$ 0.002  \\
Random$_{2.0}$     & 4.960 $\pm$ 0.004  & 0.0042 $\pm$ 0.0002 & 0.0102 $\pm$ 0.0003 & 0.450 $\pm$ 0.021  & 0.090 $\pm$ 0.002  \\
$\text{UCB}_{0}$ & 5.774 $\pm$ 0.003 & 0.0069 $\pm$ 0.0005 & 0.0154 $\pm$ 0.0007 & 0.747 $\pm$ 0.055 & 0.082 $\pm$ 0.002 \\
$\text{UCB}_{1}$ & 5.876 $\pm$ 0.003 & 0.0030 $\pm$ 0.0002  & 0.0102 $\pm$ 0.0004 & 0.338 $\pm$ 0.024 & 0.067 $\pm$ 0.002 \\
$\text{UCB}_{2}$ & 5.780 $\pm$ 0.004  & 0.0031 $\pm$ 0.0002 & 0.0093 $\pm$ 0.0003 & 0.378 $\pm$ 0.031 & 0.069 $\pm$ 0.002 \\
\midrule
\textbf{Ours}               & \textbf{6.527} $\pm$ \textbf{0.003} &\textbf{ 0.0014} $\pm$ \textbf{0.0001} & \textbf{0.0039} $\pm$ \textbf{0.0002} & \textbf{0.143} $\pm$ \textbf{0.018} &\textbf{ 0.044} $\pm$\textbf{ 0.001}
\vspace{-15pt}
\end{tabular}
}
\caption{Continuous treatments: evaluation of 40D design. More details in Appendix~\ref{sec:appendix_experiments}.} 
% \vspace{-10pt}
\label{tab:cts_40d_main}
\end{table}
% 


==> Bayesian experimental design for contextual optimisation/introduction.tex <==
\section{Introduction}\label{sec:introduction}

Machine learning models, particularly causal machine learning models, can be used to make real-world decisions \citep{joyce1999foundations,geffner2022deep}. 
We consider the problem of collecting experimental data to evaluate such models and improve decisions made in future.
For example, suppose a company has developed a model describing the relationship between customer engagement and revenue. 
This model will be used to offer personalised promotions to each customer in order to maximise some reward, e.g.~revenue.   
Before deploying it to all of its customers, % and incurring substantial costs, 
the company may wish to collect experimental data to validate the model.

To formalise this, we consider the contextual optimisation problem in which a treatment or treatments must be assigned to each context to receive a reward.
We focus on the experimental design problem of finding treatments that allow us to evaluate the regret of past actions and to improve decisions made in the future.
Our aim, then, is to choose actions to test the model; we are not directly optimising rewards in the experimental phase.
In line with our real-world scenario, we focus on designing \emph{large batch} experiments, in which we must select a large number of treatments for different contexts before receiving any feedback.

A standard experimental design procedure is random treatment assignment, which corresponds to A/B testing when treatment is binary \citep{fisher1936design,kohavi2017online}.
%, in which we apply random actions to different context members. %For a binary treatment, this corresponds to A/B testing. 
However, this naive approach has significant drawbacks, as it may involve applying many sub-optimal actions, meaning that the \emph{opportunity cost of experimentation} becomes high and experimental resources are wasted applying treatments that are known \emph{a priori} to be sub-optimal. On the other hand, applying the best treatments based on existing beliefs---a pure exploitation strategy---may also be uninformative for model testing as it fails to account for uncertainty and the need to gather data where uncertainty is high. 

To design an experiment in a more principled way, we turn to the framework of Bayesian experimental design (BED) \citep{lindley1956,chaloner1995,foster2019variational}. In contrast to standard BED, which maximises the information gained about all model parameters, we define the objective for experimental design as the \emph{expected information gained about the maximum reward obtainable for a set of evaluation contexts (max-value EIG)}.
This directly addresses the problem of gaining data to evaluate the regret of past decisions, because, given a past outcome, the unknown component of regret is \emph{how much better the reward could have been}. The formulation is also relevant to the problem of gathering data (exploration) to obtain better rewards in later interactions (exploitation). % Gathering information for regret evaluation and for model improvement are therefore two sides of the same coin.

As a model-based framework, BED requires the specification of a Bayesian model \citep{gelman2013bayesian} relating contexts, treatments and rewards. 
Since the model makes predictions about interventional distributions, causality plays a central role in selecting a correct model, particularly when the model is pre-trained with observational data.
One approach is to rely on assumptions about the causal graph \citep{pearl2009causal,sharma2021dowhy}.
Alternatively, the model can incorporate Bayesian uncertainty about the causal structure \citep{heckerman1999bayesian,annadani2021variational,geffner2022deep}.
In this paper, we propose a model-agnostic approach to experimental design that accommodates this full range of Bayesian models; we only require \emph{differentiability} of samples from the model.

To find the optimal experimental design for a given Bayesian model, we first show that the InfoNCE bound \citep{oord2018representation} can be used to estimate the max-value EIG objective.
We then optimise the testing treatment assignment (experimental design) by gradients \citep{foster2020unified,kleinegesse2020minebed}.
Our method is applicable to multiple treatments, both continuous and discrete, using carefully tuned Gumbel--Softmax \citep{maddison2016concrete,jang2016categorical} for the latter case.
We show experimentally that our approach is effective on a number of synthetic models, learning intuitively correct large batch designs that outperform standard baselines by significant margins.


% We define the objective function of an experimental design as the 


% Now start our approach 

% We adopt BOED and focus on learning max rewards

% We need a Bayesian model to use BOED and to model uncertainty.

% We need a causal model because we are predicting interventions, particularly when we combine observational and interventional data. We can also consider Bayesian uncertainty over the causal structure

% Pause


% Since treatment is an intervention, we require a model of the interventional distribution, making causal-aware models a common choice.


% We focus on model testing by evaluating the regret of some past treatments---in the real world, regret is not known because the best achievable outcomes are unknown.
% We also consider the problem of collecting data (exploration phase) to obtain better rewards in \emph{later} interactions (exploitation phase).
% These two requirements are actually two sides of the same coin---in order to correctly evaluate the regret of a past treatment assignment, we need to improve the accuracy of our estimates of the best achievable outcome for each member of the context set, and this information can also aid future treatment decisions.




% To design an experiment in a more principled way, we turn to the framework of Bayesian experimental design (BED). 
% We define the objective function of an experimental design as the expected information gained (EIG) about the maximum value obtainable for each context point. We propose a completely model-agnostic framing of this problem as one of implicit likelihood BED. 
% We show that the InfoNCE bound \citep{oord2018representation} can be used to estimate this max-value EIG.
% We optimise the testing treatment assignment (experimental design) by gradients.
% Our method is applicable to multiple treatments, both continuous and discrete, using carefully tuned Gumbel--Softmax \citep{maddison2016concrete} for the latter case.
%The method can be applied to a wide range of Bayesian models. 

%Collecting experimental data to learn optimal, context-dependent treatment assignments is a paradigm that arises in many disciplines.

% Evaluating causal inference methods is a crucially important prerequisite for their successful application in real-world decision-making tasks. 
% The development of scalable and efficient methods for causal inference evaluation, however, is an under-developed and under-explored aspect of the causal learning pipeline. 
% The standard procedure is the (multi-armed) randomized controlled trial, in which treatments (or actions) are assigned at random to a \emph{large batch} of test subjects, \textcolor{red}{each of which has a \emph{context}...}.
% For a binary treatment, this corresponds to A/B testing. 
% This naive approach has both practical and conceptual drawbacks. 
% From a practical point of view, it involves applying many sub-optimal actions, meaning that the \emph{opportunity cost} of experimentation becomes high. 
% Conceptually, we aim to learn about the best individual treatments and rewards, so gathering information about treatments which are known \emph{a priori} to be sub-optimal is not a good use of resources.
% To give a concrete example, suppose a company has developed a causal model describing the relationship between customer engagement and revenue. 
% This model will be used to offer personalized promotions to each customer in order to maximize some reward, e.g. revenue.   
% Before deploying it to all of its customers and incurring substantial costs, the company may wish to validate the learnt causal structures on a test set of customers. 

% Efficient real-world testing of causal inference methods is an important but under-explored aspect of the causal learning pipeline. For example, suppose a company has developed a causal model describing the relationship between customer engagement and revenue. 
% This model will be used to offer personalized promotions to each customer in order to maximize some reward, e.g. revenue.   
% Before deploying it to all of its customers and incurring substantial costs, the company may wish to validate the learnt causal structures on a smaller subset. 

% On the one hand,  one could run standard A/B testing to verify the learnt causal structure---a pure exploration strategy in which treatments (or actions) are applied at random, at the risk of taking many sub-optimal actions. On the other hand, one may apply treatments based on the learnt causal model---a pure exploitation strategy, \cz{which may not be so informative from model testing perspective  as one does not know what has been missed and hard to conclude if these treatment effect estimations are correct.  }which can be costly if the learnt causal associations are incorrect.



% To tackle this problem we develop BEDCITE \CZ{May want to spell the name out here}---a principled and data-efficient framework for \textbf{C}ausal \textbf{I}nference \textbf{TE}sting 
% %and \textbf{E}valuation 
% through \textbf{B}ayesian \textbf{E}xperimental \textbf{D}esign. Specifically, we define and end-to-end optimise an objective, which lower bounds the expected information gain (EIG) about the maximum value obtainable for each context point. CITeBED is scalable, model-agnostic and applicable to both continuous and discrete treatments. We demonstrate the effectiveness of our approach on \textcolor{red}{SOME models}.

% We define the objective function of an experimental design as the expected information gain (EIG) about the maximum value obtainable for each context point. Whilst existing methods generally use a fixed Bayesian model such as a Gaussian Process to solve problems of this form, we instead propose a completely model-agnostic framework that frames this problem as one of implicit likelihood Bayesian experimental design. The advantage of this approach is that we can utilise any Bayesian model (as long as it satisfies certain requirements) as the underlying model for our system. We used gradient methods to optimise the experimental treatment assignments. When the treatments are discrete, we use the Gumbel-Softmax relaxation to optimise them.


% Validating the causal models causal learning and 
% real-world decision making. 
% developing scalable and efficient methods for causal inference evaluation is  
% Real-world applications of this set-up often take the form of a small number of \emph{large batch} experiments, followed by a final deployment.
%For example, a company may wish to collect data to learn about the best promotion to offer to each of its customers in order to maximize some reward (e.g. revenue). 
%Due to the time lag between promotion and changes in business metrics, large batch experiments can be rolled out only every six months, 
%Having collected data from a handful of large batch experiments, we use it for causal structure learning and estimation of optimal treatments for the entire population.
%Such scenarios refer to learning the causal structures in (potentially very) high dimensional complex systems.


% Making optimal decisions requires (interventional) data
% Evaluating models requires data
% Consider the example of interacting with customers to find personalised optimal decisions
% We need to design large batch experiments
% A/B testing may not be optimal

% Our approach = make connection to BOED
% Reduced to problem of implicit MI maximisation
% Discrete actions
% Adaptive


==> Bayesian experimental design for contextual optimisation/method.tex <==
\begin{figure}[t]
\vspace{-20pt}
\centering
    \includegraphics[width=0.78\textwidth]{fig/figure1_U_stylized.pdf}
    \vspace{-10pt}
    \caption{An example with a scalar context and a binary treatment $\rva \in \{1,2\}$.
    The dark (resp. light) shaded area shows our uncertainty about $y|\Do{\rva},\rvc$ arising from uncertainty in $\psi$, measured by one (resp. two) st.~dev.~from the mean.
    We want to estimate $m^*=m(\rvc^*)$, the unknown maximum achievable reward at the evaluation context $\rvc^*$.
    We perform three experiments at $\rvc_1, \rvc_2, \rvc_3$ (dotted orange lines). 
    % and the mechanics of main methods. We wish to estimate $m^*=m(\rvc^*)$---the unknown maximum achievable reward in~$\rvc^*$~(dashed gray line). We can perform three experiments in $\rvc_1, \rvc_2, \rvc_3$ (dotted orange lines). 
    UCB chooses the reward-maximising treatments in each experimental context, bringing no information about $m^*$, as Treatment 2 is \emph{a priori} suboptimal at $\rvc^*$.
    Random design selects Treatments 1 and 2 with equal probability;
    our method selects treatments whose outcomes will be most informative about~$\rvm^*$ given the prior.
    \vspace{-18pt}
    }
    \label{fig:stylized_example}
\end{figure}
 
\section{Bayesian Experimental Design for Contextual Optimisation}

% \subsection{Mathematical formulation}
Whilst standard BED would design experiments to maximise the information gathered about the Bayesian parameter $\psi$, our goal is to efficiently evaluate the regret~\eqref{eq:regret}. This translates to estimating the maximum achievable rewards for a set of $D^*$ evaluation contexts $\rvC^* = \rvc^*_1,\dots,\rvc^*_{D^*}$, denoted $\rvm^* = m(\rvc^*_1),\dots,m(\rvc^*_{D^*})$.
In the customer engagement example, $\rvC^*$ represents a set of customers for which we are aiming to infer the best possible rewards $\rvm^*$.
% Since our goal is the efficient estimation of $m(c*)$ 
To learn about $\rvm^*$, we are allowed to perform a batch of $D$ experiments at contexts $\rvC = \rvc_1,\dots,\rvc_D$.
In the customer engagement example, $\rvC$ represents the set of customers that will participate in the real-world test.
% Our test contexts indicate the regions where would like to make accurate predictions of $m(\rvc)$ given the data that we will gather from the experiment.
The \emph{experimental design} problem is to select the treatments $\rvA = \rva_1,\dots,\rva_D$ to apply to $\rvC$ so that the experimental outcomes $\rvy = y_1,\dots,y_D $ that we get from the real-world test are maximally informative about $\rvm^*$.
%---the maximum rewards at the tests contexts.
More formally, we design $\rvA$ to maximize expected information gain 
% \cite[EIG,][]{lindley1956} 
between $\rvy$ and $\rvm^*$ % conditional on the contexts $\rvC$ and $\rvC^*$
% (Note: we can effectively choose which partners to experiment on as well by choosing a large experiment set, and setting some actions to `no action'.)
% Our approach can be summarised as applying Bayesian experimental design by designing $\rvA$ to maximise 
\begin{align}
    \mathcal{I}(\rvA; \rvC, \rvC^*) %
    %&= \E_{\unconditionaljoint} 
    %\left[ 
    %    \log \frac{\unconditionaljoint}{ p(\rvy|  \rvC, \Do{\rvA})p(\rvm^*|\rvC^*) } 
   % \right] \\
        % &= \E_{p(\psi)p(\rvy, \rvm^* | \rvC, \rvC^*, \Do{\rvA}, \psi)} 
    % \left[ 
    %     \log \frac{ p(\rvm^*) p(\rvy |\rvm^*, \Do{\rvA},  \rvC) }{ p(\rvy|\Do{\rvA},  \rvC)p(\rvm^*) }
    % \right] \nonumber \\
    &= \E_{\unconditionaljoint}  %{p(\psi)p(\rvy, \rvm^* | \rvC, \rvC^*, \Do{\rvA},  \psi)} 
    \left[ 
        \log \frac{  p(\rvy |\rvm^*, \Do{\rvA},  \rvC) }{ p(\rvy|\Do{\rvA},  \rvC) }
    \right], \label{eq:mi_objective}
\end{align}
where $p(\rvy|\Do{\rvA},  \rvC) = \E_{p(\psi)} \big[ p(\rvy|\Do{\rvA},  \rvC, \psi) \big]$, $p(\rvm^* | \rvC^*) = \E_{p(\psi)} \big[p(\rvm^* | \rvC^*, \psi)\big]$ and $\unconditionaljoint = \E_{p(\psi)} \big[ p(\rvm^* | \rvC^*, \psi) p(\rvy | \rvC, \Do{\rvA}, \psi) \big]$. 
% Note that $\mathcal{I}(\rvA; \rvC, \rvC^*)$ is equal to the mutual information between the quantity of interest $\rvm^*$, and the outcomes $\rvy$ given the context $\rvC$ when performing experiment $\rvA$. 
We refer to $\mathcal{I}(\rvA; \rvC, \rvC^*)$ as the max-value EIG.
The objective is doubly intractable \citep{rainforth2018nesting} meaning that its optimisation, or even evaluation with a fixed $\rvA$, is a major challenge. The likelihoods in the expectation are \emph{implicit} (not available analytically) making the problem more difficult. % In such cases one often relies on non-scalable gradient-free methods, e.g. Bayesian optimisation \citep{kleinegesse2019efficient}.

% We wish to find the optimal designs by maximising \eqref{eq:mi_objective}, i.e. $\rvA^* = \argmax_A \mathcal{I}(\rvA)$, with gradients. % By assumption, we have a powerful simulator which can get us samples from the joint
% Unfortunately, the expression inside the expectation is not available in closed form, so in this section we look at ways to approximate it.  

% \begin{align} 
%     \unconditionaljoint &= \E_{p(\psi)} \big[  \conditionaljoint \big] \\
%                         &= \E_{p(\psi)} \big[ p(\rvm^* | \rvC^*, \psi) p(\rvy | \rvC, \Do{\rvA}, \psi) \big]
% \end{align}
% \begin{equation}
%     \mathcal{I}(\rvA; \rvC, \rvC^*) = \E_{p(\psi)\conditionaljoint} 
%     \left[ 
%         \log \frac{ \unconditionaljoint }{ p(\rvy|  \rvC, \Do{\rvA})p(\rvm^*|\rvC^*) }
%     \right] \label{eq:mi_objective}
% \end{equation}


%\begin{itemize}
    % \item The \emph{conditional on $\psi$} joint $p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA}, \psi)$ is given by
    %     \begin{align}
    %         p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA}, \psi) &= p(\rvm^* | \rvC^*, \psi) p(\rvy | \rvm^*, \rvC, \rvC^*, \Do{\rvA}, \psi) \\
    %         & = p(\rvm^* | \rvC^*, \psi) p(\rvy | \rvC, \Do{\rvA}, \psi)
    %     \end{align}
    %     Conditional on $\psi$ we can draw samples $y | c, \Do{a}$ and $\rvm^* | \rvc^*, \psi$ (which is deterministic and equals $m(c^*; \psi)$)
    %%
    % \item Unconditional joint, $p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA})$:
    %     \begin{align}
    %         p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA}) &= \E_{p(\psi)} \big[ p(\rvy,\rvm^* | \rvC, \rvC^*, \Do{\rvA}, \psi) \big]
    %     \end{align}
    %%
    % \item The marginal $p(\rvm^* | \rvC^*)$
    %     \begin{equation}
    %             p(\rvm^* | \rvC^*) = \E_{p(\psi)} \big[p(\rvm^* | \rvC^*, \psi)\big] = \int_\psi p(\psi) p(\rvm^* | \rvC^*, \psi)d\psi 
    %     \end{equation}
    %     and since $m^* | \psi$ is deterministic, $p(m^*|\psi) = \delta(m^*=m(c^*;\psi))$
    %%
    % \item Marginal outcome
    %     \begin{equation}
    %         p(\rvy|\Do{\rvA},  \rvC) = \E_{p(\psi)} \big[ p(\rvy|\Do{\rvA},  \rvC, \psi) \big]  
    %     \end{equation}
%\end{itemize}   



\subsection{Training stage: Objective estimation and optimization}\label{sec:training_stage}

Recently, gradient-based approaches for optimising EIG %\eqref{eq:mi_objective} 
have been developed for experimental design for parameter learning \citep{foster2020unified, kleinegesse2020minebed} as opposed to contextual optimisation, which is the focus of this work. 
Inspired by likelihood-free mutual information estimators, we show the InfoNCE bound \citep{oord2018representation} can be adapted to the contextual optimisation setting we consider here. Concretely,
%\vspace{-5pt}
\begin{equation}
% \vspace{-6pt}\hspace{-7pt}
    \mathcal{L}(\rvA, U; \rvC, \rvC^*, L) = \E_{p(\psi)p(\rvy, \rvm^*_0 | \Do{\rvA},  \rvC, \rvC^*, \psi)p(\rvm^*_{1:L}| \rvC^*)} 
    \left[ 
        \log \frac{  \exp(U(\rvy , \rvm^*_0))}{ \frac{1}{L+1} \sum_\ell \exp(U(\rvy , \rvm^*_\ell)) }
    \right] \label{eq:infonce_bound}
\end{equation}
is a lower bound on~$\mathcal{I}(\rvA;\rvC,\rvC^*)$ for any $L \geq 1$ and any critic function $U$. We provide a proof of this claim in Appendix~\ref{sec:appendix_proofs}. To learn a suitable critic $U$, we use a neural network with trainable parameters $\phi$.
We then optimise the lower bound $\mathcal{L}(\rvA, U; \rvC, \rvC^*, L)$ simultaneously with respect to $\phi$ and $\rvA$, thereby improving the tightness of the bound and optimising the experimental design together.
When the actions $\rvA$ are continuous, we require that a sample $y$ of $p(y|\Do{\rva},\rvc,\psi)$ is differentiable with respect to $\rva$. 
In this case, a pathwise gradient estimator \citep{mohamed2020monte} for $\nabla_{\rvA, \phi}\mathcal{L}$ can be readily computed and we apply standard stochastic gradient ascent (SGA) \citep{robbins1951stochastic} to optimise our objective~\eqref{eq:infonce_bound}.


%To this end, we introduce a trainable function $U_\phi$ which takes $y$-s and $m^*$-s as inputs (recall we get these from our simulator), and outputs a real number.  The InfoNCE \citep{oord2018representation} lower bound on the Mutual Information in \eqref{eq:mi_objective} is 



%In practice, we will parametrise $U_\phi$ by a neural network with trainable parameters $\phi$; we can then easily obtain an unbiased estimate of \eqref{eq:infonce_bound} using samples from our simulator, and also back-propagate using standard auto-differentiation software. Assuming a \emph{continous action space}, we can optimse $\mathcal{L}$ with respect to $\rvA$ and $\phi$ jointly.


%For a given $\psi$, we can sample theoretical experimental outcomes $y_1,\dots,y_D | \rvc_1,\dots,\rvc_D,\text{do}(\rva_1,\dots,\rva_D),\psi$ and the maximum values for our test set $m(\rvc^*_1),\dots,m(\rvc^*_{D^*})|\psi$. 



\paragraph{Discrete action space}
% To deal with discrete actions, we introduce a parametrized policy ...  
Previous gradient-based BED work has focused on fully differentiable models. 
Here we propose a practical way to deal with discrete designs. % by applying the Gumbel--Softmax \citep{maddison2016concrete, jang2016categorical} relaxation. 
%Concretely, instead of optimising over $\rvA$ directly, we represent it as 
% Suppose there are $K$ possible treatments we can choose from per design $\rva$. 
Rather than learning the treatments $\rvA$ directly, we introduce a stochastic treatment policy $\pi_{\bm{\alpha}}$ with trainable parameters $\bm{\alpha}$ representing the probabilities of selecting each treatment. % The final treatment assignment is sampled $\rvA\sim \pi_{\bm{\alpha}}$. However, 
During training we use a Gumbel--Softmax \citep{maddison2016concrete, jang2016categorical} relaxed form of $\rvA$ and update $\bm{\alpha}$ by gradients.
% At a high level this involves learning a stochastic policy $\pi_\alpha$ with trainable parameters $\alpha$, representing the probabilities of selecting each treatment.  
Further detail is provided in Appendix~\ref{sec:appendix_proofs}.

\subsection{Deployment stage: Real-world testing}\label{sec:deployment}
Once we optimise the objective~\eqref{eq:infonce_bound}, we perform the batch of experiments $\rvA$ to obtain real-world outcomes $\rvy$ and estimate $p(\psi|\mathcal{D})$---the posterior of our Bayesian model, given the experimental data $\mathcal{D}=(\rvy, \rvA, \rvC)$.
We then calculate the posterior $p(\rvm^*|\rvC^*,\mathcal{D})$, and this it to estimate the regret~\eqref{eq:regret} of a set of past treatments.
Importantly, through our design of $\rvA$, the data contained in $\mathcal{D}$ should lead to the \emph{most accurate} estimate of $\rvm^*$, which translates to an accurate estimate of the regret and an accurate evaluation metric for the original decisions.
% In other words, the posterior distribution $p(\rvm^*|\rvC^*,\mathcal{D})$ should have low uncertainty.
% 
% This updated model should then give us accurate estimates of $\rvm^*$,
% the maximum obtainable reward at each of our evaluation contexts. $\rvC^*$.
% A complete high level description of our framework  in 
Algorithm \ref{algo:method} in the Appendix gives a complete description of our method. 


==> Bayesian experimental design for contextual optimisation/relwork.tex <==
\section{Related Work}
% 1 MES/PES, 2 contextual BO, 3 contextual bandits (particularly this emma brunskill paper),
% 4 our/Gutmann's existing work on implicit BED.
% , I think we want four paragraphs: 1 MES/PES, 2 contextual BO, 3 contextual bandits (particularly this emma brunskill paper), 4 our/Gutmann's existing work on implicit BED.
% Our work is connected to three broad frameworks---Bayesian Optimisation, Bayesian experimental design  and contextual bandits.
The most closely related objective to our max-value EIG \eqref{eq:mi_objective} is Max-value Entropy Search \citep[MES,][]{wang2017max}. It was proposed as a computationally efficient alternative to Entropy Search \citep[ES,][]{hennig2012entropy} and Predictive Entropy Search \citep[PES, ][]{hernandez2014predictive}. Our objective %~\ref{eq:mi_objective} and the associated lower bound~\ref{eq:infonce_bound} 
differs from MES in two essential ways: firstly, MES is applicable to Gaussian processes (GPs), whilst our objective is model-agnostic; secondly, we focus on \emph{contextual} optimisation, rather than finding a single maximiser. For a more comprehensive discussion of related work, see Appendix~\ref{sec:app:relwork}.



